Planes in four space and four associated CM points

To any two-dimensional rational plane in four-dimensional space one can naturally attach a point in the Grassmannian Gr(2,4) and four lattices of rank two. Here, the first two lattices originate from the plane and its orthogonal complement and the second two essentially arise from the accidental local isomorphism between SO(4) and SO(3)xSO(3). As an application of a recent result of Einsiedler and Lindenstrauss on algebraicity of joinings we prove simultaneous equidistribution of all of these objects under two splitting conditions.

==> old.tex <==
\newpage












%\begin{proposition}[A suitable basis]
%Let $\Lambda$ be the set of $\Z$-points of a rational plane in $\R^4$. Then there is a basis $v_1,v_2$ of $\Lambda$, vectors $w_1,w_2 \in \Z^4$ and a basis $u_1,u_2$ of $L^\perp \cap \Z^4$ so that
%\begin{align*}
%g_L := (u_1,u_2,w_1,w_2) \in \SL_4(\Z).
%\end{align*}
%and $(w_i,v_j) = \delta_{ij}$ for $i,j=1,2$. 
%\end{proposition}
%\subsection{Packets under rank two torus action}


%\begin{proof}
%Let the columns of $X\in \Mat_{4,2}(\Z)$ consist of an arbitrary basis of $\Lambda$. Apply the elementary divisor theorem to obtain $S \in \SL_4(\Z)$ and $T \in \SL_2(\Z)$ such that
%\begin{align*}
%SXT = \begin{pmatrix}
%\alpha_1 &  \\ 
% & \alpha_2 \\ 
% &  \\ 
% & 
%\end{pmatrix} = X'
%\end{align*}
%with $\alpha_1 | \alpha_2$. We claim that $\alpha_1 = \alpha_2 = 1$ by maximality of $\Lambda$ (as a integral lattice in the plane it spans). Indeed, note that otherwise $\Lambda$ is strictly contained in 
%\begin{align*}
%S^{-1} \begin{pmatrix}
%1 &  \\ 
% & 1 \\ 
% &  \\ 
% & 
%\end{pmatrix} T^{-1} \Z^2.
%\end{align*}
%Set $v_i = gTe_i \in L$, $w_i = S^t e_i$ and $u_i = S^t e_{i+2}$ for $i = 1,2$. Compute
%\begin{align*}
%(w_i,v_i) = e_i^t g' e_i = 1, \quad (u_i,v_j) = ... =  0.
%\end{align*}
%This implies that $u_1,u_2$ is a basis of $\Lambda^t \cap \Z^4$.
%\end{proof}




%\newpage
%
%\section{Orbital setup}
%
%Let $Q$ and $\iota_Q$ be as before and set $L := \iota_Q(\Z^2)$ and $\mathbb{H} = \mathbb{H}_{Q,\iota_Q}$ for simplicity.
%
%\subsection{Reproducing integral embeddings}
%
%\begin{claim}
%The orbit $\BH(\adele)\G_1(\Q) $ is closed in $\rquot{\G_1(\adele)}{\G_1(\Q)}$.
%\end{claim}
%
%\begin{proof}
%We do this explicitly even though a reference would probably suffice. Consider a sequence $h_k \in \BH(\adele)$ and $\gamma_k \in \G_1(\Q)$, so that $h_k \gamma_k \to g \in \G(\R \times \hat{\Z})$. Let $z \in L$ be a point. Then the sequence $\gamma_k^{-1}h_k^{-1}z = \gamma_k^{-1}z \in \Q^4$ is convergent and hence eventually constant. For large enough $k$ we thus have $\gamma_k^{-1}z = g^{-1}z$. Choose $k$ large enough so that $\gamma_k^{-1}e_i = g^{-1}e_i$, where $e_1,e_2$ is a basis of $L$. Then $\gamma_k^{-1}z = g^{-1}z$ for all $z \in L$ and $g\G_1(\Q) \in \BH(\adele) \G_1(\Q)$. 
%\end{proof}
%
%
%Write for simplicity $\Gamma = \G_1(\Q)$. Let $ g^{-1} \Gamma \in \BH(\adele)\G_1(\Q) $ where $g \in \G_1(\R \times \hat{\Z}) $ and $g h = \gamma \in \Gamma$ where $h \in \BH(\adele)$. Then
%\begin{align*}
%(\R \times \hat{\Z})^4 \supset g  L = g h L = \gamma L \subset \Q^4
%\end{align*}
%and in particular $ \gamma L \subset \Z^4$. Therefore, $\gamma \circ \iota_Q$ is again a representation of $Q$ by $Q_0$.
%
%\begin{lemma}
%$\gamma \circ \iota_Q$ is a primitive representation of $Q$.
%\end{lemma}
%
%\begin{proof}
%TO DO.
%\end{proof}
%
%\begin{lemma}
%$\gamma \circ \iota_Q$ is equal to $\iota_Q$ modulo $\G_1(\Z)$ if and only if their are in the same orbit.
%\end{lemma}
%
%\begin{proof}
%TO DO.
%\end{proof}
%
%Note that the group $ \BH(\R \times \hat{\Z})$ acts on $\BH(\adele)\G_1(\Q) $ from the left. We may write
%\begin{align*}
%\BH(\adele)\G_1(\Q)  = \Disjointunion_{\rho \in \CR} \BH(\R \times \hat{\Z})\rho\Gamma.
%\end{align*}
%by compactness for a finite set of representatives $\CR \subset \BH(\R \times \hat{\Z})$. Note that the cardinality of $\CR$ is naturally the class number of $\BH$. This will be used to derive a asymptotic counting statement for $|\CR|$ as $D$ gets large. Let $S$ be the set of places $\set{\infty,p,q}$, where $p,q$ are two distinct odd primes. There is a well-defined projection onto the $p$-adic extension
%\begin{align*}
%\pi_{p,\infty}: \rquot{\G_1(\adele)}{\G_1(\Q)} \to   \rquot{\G_1(\Q_S)}{\G_1(\Z^S)} =: X_S
%\end{align*}
%where $p$ is an arbitrary prime. The analogous statement is true for the real extension. The projection of the adelic orbit of $\BH$ onto the $p$-adic extension is
%\begin{align}\label{eq:first attempt at orbits}
%\Disjointunion_{\rho \in \CR} \BH(\Z_S) (\rho_\infty,\rho_p,\rho_q) \G_1(\Z^S)
%\end{align}
%
%\subsubsection{About the stabilizer}
%
%In the following, we will assume that $p$ is an odd prime and that $p \nmid D$. By definition, $\BH$ may be seen as the (special) orthogonal group of $Q_0$ restricted to $L^\perp$.  Since the discriminant of $Q$ is $D$, the same is true for the binary form $Q_0|_{L^\perp}$. By REF we deduce
%
%\begin{proposition}
%The following are equivalent:
%\begin{enumerate}[(i)]
%\item The group $\BH(\Qp)$ is split.
%\item $-D$ is a square mod $p$.
%\end{enumerate}
%\end{proposition}
%
%We now strengthen this and include the $\Zp$-points of $\BH$ into the discussion. To do so, we make use of Lemma 2.8 in REF, Thesis and deduce that 
%
%\begin{proposition}
%If $-D$ is a square mod $p$, then there exists a $\Zp$-basis of $\Zp^4$, on which $Q_0$ takes the form
%\begin{align*}
%x_1x_2+x_3x_4
%\end{align*}
%i.e. is of signature (2,2).
%\end{proposition}
%
%Upon conjugating \eqref{eq:first attempt at orbits} over $\Zp$, we thus obtain for any $D$ satisfying Linnik's condition for $p$ and $q$ an $\BH(\Q_S)$-invariant collection of orbits
%\begin{align*}
%\Disjointunion_{\rho \in \CR_D} \BH(\Z_S) \rho \G_1(\Z^S) =: \mathcal{O}_D
%\end{align*}
%where $\BH$ does not(!) depend on $D$.
%
%\begin{conjecture}[Equidistribution of collection of orbits on $\SU_2^2$-quotient]\label{conj:Equidistribution of collection of orbits on SU_2^2-quotient}
%The Haar measures $\mu_D$ on $\mathcal{O}_D$ equidistribute to the Haar measure on $X_S$ as $D_\to \infty$ with $D\in \mathbb{D}$ and $D$ satisfying Linnik's condition for $p$ and $q$.
%\end{conjecture}
%
%Note that this conjecture rather immediately implies Conjecture \ref{conj:equidistribution of planes}.
%
%\newpage
%\section{Reformulation in order to use joinings}
%
%%In this section we would like to formulate and prove a precise version of the following proposition:
%%
%%\begin{proposition}
%%Conjecture \ref{conj:Equidistribution of collection of orbits on SO_4-quotient} follows from a conjecture concerning equidistribution on the product space $\rquot{\SO_3(\Q_S)}{\SO_4(\Z^S)}$ with itself.
%%\end{proposition}
%%
%%Denote by $D_1$ the norm one quaternions and recall that $D_1 = \SU_2$. The map 
%%\begin{align}
%%\phi: D_1 \times D_1 \to \SO_4 = \G_1, \quad (\alpha,\beta) \mapsto (x \mapsto \alpha x \beta^{-1})
%%\end{align}
%%is a surjective isogeny with kernel $ \set{(1,1),(-1,-1)}$. We thus obtain an injective map
%%\begin{align*}
%%\bar{\phi}: X_S' := \rquot{\SU_2\times \SU_2(\Q_S)}{\phi^{-1}(\SO_4(\Z^S))} \hookrightarrow \rquot{\SO_4(\Q_S)}{\SO_4(\Z^S)} = X_S
%%\end{align*}
%%As the image of $\SU_2\times \SU_2(\Q_S)$ in $\SO_4(\Q_S)$ is open, the image of $\bar{\phi}$ is also open. By compactness we may write the space
%%\begin{align*}
%%\rquot{\SO_4(\Q_S)}{\SO_4(\Z^S)}
%%\end{align*}
%%as a finite union of translated images of $\bar{\phi}$. For concreteness, we write
%%\begin{align*}
%%X_S = \bigsqcup_{g \in \mathcal{G}} g \bar{\phi}(X_S'),
%%\end{align*}
%%where $\mathcal{G} \subset \SO_4(\Z_S)$ is a finite set. In particular, we obtain
%%
%%\begin{lemma}
%%The collections $\mathcal{O}_D$ equidistribute if and only if the collections $\bar{\phi}^{-1}(\mathcal{O}_D)$ do so.
%%\end{lemma}
%%
%%Furthermore, considering the surjection
%%\begin{align*}
%%\bar{\phi}_1:\rquot{\SU_2\times \SU_2(\Q_S)}{\SU_2\times \SU_2(\Q_S)} \to \rquot{\SU_2\times \SU_2(\Q_S)}{\phi^{-1}(\SO_4(\Z^S))}
%%\end{align*}
%%yields
%
%
%
%
%
%%By standard arguments $\phi$ is surjective on $\R$-points. We show by brute force, that it is also surjective on $\Qp$-points for any $p$.
%%
%%\begin{proposition}
%%The map $ \phi: D_1(\Qp) \times D_1(\Qp) \to \SO_4(\Qp)$ is surjective.
%%\end{proposition}
%%
%%\begin{proof}
%%Since $D_1 \times D_1$ acts transitively on norm one elements and the stabilizer of $1$ is the diagonal subgroup $D_1 < D_1 \times D_1$, we see that it suffices to show that the induced map $\psi: D_1(\Qp) \to \SO_3(\Qp),\ \alpha \mapsto (x \mapsto \alpha x \alpha^{-1})$ is surjective. However, notice that the action is exactly the adjoint action of $\SU_2(\Qp)$ on its Lie algebra. The proposition thus follows from the following claim.
%%\end{proof}
%
%\subsection{From integral lattices to pairs of integer points}
%
%In this subsection, we aim to prove the following proposition and some consequences. Recall first that the trace $\Tr$ of a quaternion is defined as the sum of the quaternion and its conjugate. Furthermore, the norm $Q_0$ is the product of the quaternion and its conjugate. In particular, for any quaternion $q$ we have
%\begin{align*}
%Q_0(q) = q\overline{q} = \frac{1}{2}\Tr(q+\overline{q}).
%\end{align*}
%Thus, the standard inner product is given by
%\begin{align*}
%\frac{1}{2}(Q_0(q_1+q_2)-Q_0(q_1)-Q_0(q_2)) = \frac{1}{2}(q_1\overline{q_2}+q_2 \overline{q_1}) = \frac{1}{2}\Tr(q_1\overline{q_2}).
%\end{align*}
%
%
%\begin{proposition}\label{prop:assoc.int.pairs}
%Let $L$ be a rank $2$ sublattice of $\Z^4$ of discriminant $D$ and let $(\alpha_1,\alpha_2) \in \SU_2^2$ be in the stabilizer of $L$. Let $v_1,v_2\in L$ be a $\Z$-basis. Then the points
%\begin{align*}
%u_1 := v_2\overline{v_1} - \frac{1}{2}\Tr(v_2\overline{v_1})\\
%u_2 := \overline{v_2}v_1 - \frac{1}{2}\Tr(\overline{v_2}v_1)
%\end{align*}
%are traceless, integral, of length $D$ and are stabilized under conjugation by $\alpha_1,\alpha_2$ respectively.
%\end{proposition}
%
%\begin{proof}
%By definition $u_1,u_2$ are traceless and integral. Furthermore, we have for $i \in \set{1,2}$ the condition
%\begin{align*}
%\alpha_1 v_i \alpha_2^{-1} = v_i.
%\end{align*}
%We compute
%\begin{align*}
%\alpha_1 v_2\overline{v_1} \alpha_1^{-1} =  v_2\alpha_2\overline{v_1} \alpha_1^{-1} = v_2 \overline{\alpha_1v_1\alpha_2^{-1}} = v_2 \overline{v_1}
%\end{align*}
%and analogously
%\begin{align*}
%\alpha_2\overline{v_2}v_1 \alpha_2^{-1} = \alpha_2\overline{v_2}\alpha_1^{-1}v_1 = \overline{v_2}v_1,
%\end{align*}
%which proves that $u_1,u_2$ are stabilized under conjugation by $\alpha_1,\alpha_2$ respectively. It remains to show that $u_1$ and $u_2$ are of length $D$. We compute
%\begin{align*}
%u_1 \overline{u_1} 
%&= (v_2\overline{v_1} - \frac{1}{2}\Tr(v_2\overline{v_1})(v_1\overline{v_2} - \frac{1}{2}\Tr(v_2\overline{v_1})\\ 
%&= Q_0(v_1)Q_0(v_2) + \frac{1}{4}\Tr(v_2\overline{v_1})^2 - \frac{1}{2}\Tr(v_2\overline{v_1}) (v_2\overline{v_1}+v_1 \overline{v_2})\\
%&= Q_0(v_1)Q_0(v_2) - \frac{1}{4}\Tr(v_2\overline{v_1})^2 \\
%u_2 \overline{u_2} &= (\overline{v_1}v_2 - \frac{1}{2}\Tr(\overline{v_2}v_1))(\overline{v_2}v_1 - \frac{1}{2}\Tr(\overline{v_2}v_1)) \\
%&= Q_0(v_1)Q_0(v_2) - \frac{1}{4}\Tr(\overline{v_1}v_2)^2 = u_1 \overline{u_1} 
%\end{align*}
%and compare this to the discriminant of $L$. In the basis $v_1,v_2$ the quadratic form $Q_0|_L$ is given by
%\begin{align*}
% Q_0(v_1)x^2 - \Tr(v_1\overline{v_2})xy +  Q_0(v_2)y^2
%\end{align*}
%and thus the discriminant is equal to $u_1 \overline{u_1} = u_2 \overline{u_2}$.
%\end{proof}
%
%\begin{lemma}
%Let $L$ be as in the proposition. The integer points in $\Z^3$ generated from $L$ depend on the choice of basis only up to a sign.
%\end{lemma}
%
%\begin{proof}
%Let $v_1,v_2$ be a basis of $L$ and let $A\in \GL_2(\Z)$. Note that the map 
%\begin{align*}
%f: (u,v) \mapsto v\overline{u}-\Tr(v\overline{u})
%\end{align*}
%is antisymmetric and bilinear. Hence,
%\begin{align*}
%f(a_{11}v_1+a_{12}v_2,a_{21}v_1+a_{22}v_2) &= a_{11}a_{22}f(v_1,v_2)+ a_{12}a_{21}f(v_2,v_1)\\ &= \det(A) f(v_1,v_2)
%\end{align*}
%which concludes the claim for $u_1$. Everything is analogous for $u_2$.
%\end{proof}
%
%We shall call the pair $(u_1,u_2)$ the \textbf{integer pair associated to $L$} and denote it by $(v(L)_1,v(L)_2)$. 
%
%%If $v_1,v_2$ is a basis of a lattice $L$, then\note{to correct yet.}
%%\begin{align*}
%%v(L)_1 = v_2 v(L)_2 v_2^{-1}
%%\end{align*}
%%and vice versa as a quick computation shows.
%
%
%%\begin{remark}[Remaining questions]
%%$ $
%%\begin{enumerate}
%%\item Are the integer points $\R^3$ generated from $L$ primitive, if $L$ is primitive? Maintaining the square-free assumption, the integer pair associated to $L$ is certainly primitive. In general this may not be true, use SAGE to find a (possible) counterexample.
%%\item Can one say anything about the angle between the integer points in $\R^3$ generated from $L$?
%%\item Is the correspondence one to one? Definitely not (at least not with the obvious range) by counting problems.
%%\end{enumerate}
%%\end{remark}
%
%We now discuss an alternative way to construct the associated integer pair. To do so, notice that the maps
%\begin{align*}
%(u,v) \mapsto v\overline{u}-\Tr(v\overline{u}),\quad (u,v) \mapsto \overline{v}u-\Tr(\overline{v}u)
%\end{align*}
%factor through $\bigwedge^2 \Q^4 \cong \Q^6$, where the isomorphism is induced by the choice of basis $1 \wedge i,\ 1\wedge j,\ 1 \wedge k,\ i\wedge j,\ i \wedge k,\ j \wedge k$. Therefore one obtains the induced maps
%\begin{align*}
%x \mapsto  \begin{pmatrix}
%x_{12}+x_{34} \\ 
%x_{13}-x_{24} \\ 
%x_{14}+x_{23}
%\end{pmatrix},\quad
%x \mapsto  \begin{pmatrix}
%-x_{12}+x_{34} \\ 
%-x_{13}-x_{24} \\ 
%-x_{14}+x_{23}
%\end{pmatrix}.
%\end{align*}
%and hence an alternative formula for the associated integer pair. In particular, the integer pair associated to a lattice uniquely determines the lattice. In fact, if $L$ is a primitive lattice, $v_1,v_2$ is a basis and $x = v_1 \wedge v_2$, then  $x \wedge x = 0$ which yields in our choice of basis
%\begin{align*}
%x_{12}x_{34}-x_{13}x_{24}+x_{14}x_{23} = 0.
%\end{align*}
%We shall now use these observations to describe the splitting field of the $\Q$-torus $\BH_{L}$. Recall
%
%%\begin{lemma}\label{lemma:splittingfield for point.stab.}
%%Let $v\in \Z^3$ be a primitive integer point of length $d$ and let $\BH_v < \SU_2$ be the stabilizer of $v$. Then the splitting field of $\BH_v$ is $\Q(\sqrt{-d})$ and there is $g \in \SU_2(\Q(\sqrt{-d}))$ such that
%%\begin{align*}
%%g\BH_vg^{-1} = \BH_{gv} = \set{\begin{pmatrix}
%%* & 0 \\ 
%%0 & *
%%\end{pmatrix} } < \SU_2
%%\end{align*}
%%\end{lemma}
%%
%%\begin{proof}
%%TO DO.
%%\end{proof}
%%
%%We now the above lemma to show that $\BH_L$ also has splitting field $\Q(\sqrt{-d})$. Let $(g,h) \in \SU_2(\Q(\sqrt{-d}))$ be so that $g\BH_{v(L)_1}g^{-1}$ and $h\BH_{v(L)_2}h^{-1}$ are diagonal as Lemma \ref{lemma:splittingfield for point.stab.}. Consider the plane $(g,h).L$. If $v_1,v_2$ are a basis for $L$ then $(g,h).v_1$ and $(g,h).v_2$ form a basis of $L$. Therefore, the integer points associated to $L$ are up to scalars
%%\begin{align*}
%%\left(gv_2h^{-1}\right)\overline{\left(gv_1h^{-1}\right)}-\tfrac{1}{2}\Tr(\left(gv_2h^{-1}\right)\overline{\left(gv_1h^{-1}\right)})
%%= g.v(L)_1
%%\end{align*}
%%and $h.v(L)_2$. In particular, the plane $(g,h).L$ has the same associated points as the plane $\text{span}(1,\mathrm{i})$ and thus $(g,h).L = \text{span}(1,\mathrm{i})$. We deduce that
%%\begin{align*}
%%(g,h) \BH_L (g,h)^{-1} = \BH_{(g,h).L} = \setc{(g',g')}{g' = \begin{pmatrix}
%%* & 0 \\ 
%%0 & *
%%\end{pmatrix} \in \SU_2 } < \SU_2^2.
%%\end{align*}
%
%\subsection{A correspondence}
%
%\begin{proposition}
%Let $D\in \N$ be fixed (possibly squarefree). There is a one-to-one correspondence 
%\begin{align*}
%\setc{\Lambda \subset \Z^4}{\Lambda \text{ primitive with discriminant }d}
%\longleftrightarrow
%\setc{v \in \Z^3}{\norm{v}_2^2 = D}^2
%\end{align*}
%given by $\Lambda \mapsto (v(\Lambda)_1,v(\Lambda)_2)$. In particular, the cardinality of either set is $D^{1+o(1)}$ if $D$ satisfies Legendre's condition.\note{Maybe there are finite index issues.}
%\end{proposition}
%
%\begin{proof}
%Let $\Lambda$ be a primitive sublattice of $\Z^4$ with discriminant $D$ and let $v_1,v_2$ be a basis of $\Lambda$. We first recall that the integer pair of $\Lambda$ is given by the formulas
%\begin{align*}
%v(\Lambda)_1 := v_2\overline{v_1} - \tfrac{1}{2}\Tr(v_2\overline{v_1})\\
%v(\Lambda)_2 := \overline{v_2}v_1 - \tfrac{1}{2}\Tr(\overline{v_2}v_1)
%\end{align*}
%up to signs. Note that in particular the relations
%\begin{align}\label{eq:relationbasisvsintpts}
%v(\Lambda)_1\cdot v_2 = v_2\cdot v(\Lambda)_2, \quad
%v(\Lambda)_2\cdot v_1 = v_1\cdot v(\Lambda)_1
%\end{align}
%hold. Further, observe that for any $g,h \in \SU_2$
%\begin{align*}
%&v(\Lambda h)_1 = v(\Lambda)_1,\quad v(g\Lambda)_1 = g v(\Lambda)_1g^{-1} \\
%&v(g\Lambda)_2 = v(\Lambda)_2,\quad v(\Lambda h)_2 = h^{-1} v(\Lambda)_1h.
%\end{align*}
%
%\textsc{Claim.} The associated integer points uniquely determine the lattice $\Lambda$.
%
%Let $\Lambda'$ be another primitive sublattice of $\Z^4$ with discriminant $D$ and assume that $v(\Lambda)_i = v(\Lambda')_i$ for $i=1,2$. Choose $(g,h) \in \SU_2(\R)^2$ so that
%\begin{align*}
%g (\Lambda \otimes \R) h^{-1} = \langle 1,\mathrm{i} \rangle_{\R}
%\end{align*}
%and let $L = g (\Lambda' \otimes \R) h^{-1}$. It suffices to show that $L = \langle 1,\mathrm{i} \rangle_{\R}$. Note that changing the lattice $g \Lambda' h^{-1}$ to another lattice in $L$ only changes the corresponding point in $\R^3 \times \R^3$ by a multiple (the discriminant). 
%We have thus reduced the claim to showing that any lattice $\tilde{\Lambda}$ with $v(\tilde{\Lambda})_1 = v(\tilde{\Lambda})_2 = \mathrm{i}$ is contained in $\langle 1,\mathrm{i} \rangle_{\R}$. 
%Let $v_1,v_2$ be a basis of $\tilde{\Lambda}$.
%By Equation \ref{eq:relationbasisvsintpts} we have
%\begin{align*}
%\mathrm{i} v_2 = v_2 \mathrm{i},\quad \mathrm{i} v_1 = v_1 \mathrm{i}.
%\end{align*}
%This proves the claim.
%
%We now change perspective somewhat. Let $x_1,x_2$ be two primitive integer points in $\Z^3$ of length $\sqrt{d}$, which we identify as usual with tracefree quaternions. Define
%\begin{align*}
%\mathbb{T}_1 = \Stab_{\SU_2}(x_1),\quad \mathbb{T}_2 = \Stab_{\SU_2}(x_2).
%\end{align*}
%As both these tori are maximal $\Q$-tori, there exists $g \in \SU_2(\Q)$ with
%\begin{align*}
%g \mathbb{T}_1 g^{-1} = \mathbb{T}_2.
%\end{align*}
%In particular, $g.x_1 \Vert x_2$. As $g$ acts as an orthogonal transformation we may replace $x_2$ by $-x_2$ if necessary so that $g.x_1 = x_2$.\note{Here$->$ finite index (everything is projective)} The natural candidate for a lattice $\Lambda$ with integer pair $(x_1,x_2)$ is now given by the $\Z$-points of
%\begin{align*}
%\setc{v}{ \forall t \in \mathbb{T}_1: tv (gtg^{-1}) = v}
%&= \setc{v}{ \forall t \in \mathbb{T}_1: t (vg) = (vg)t} \\
%&= \setc{w}{ \forall t \in \mathbb{T}_1: t w = wt}g^{-1}.
%\end{align*}
%Note that the rational plane $\setc{w}{ \forall t \in \mathbb{T}_1: t w = wt}g^{-1}$ is two-dimensional and let $\Lambda$ be defined as above. It remains to show that the integer pair associated to $\Lambda$ is indeed given by $(x_1,x_2)$. To see this, note that $v(\Lambda)_1$ is stabilized by all $t \in \mathbb{T}_1$ and the analogous statement holds for $v(\Lambda)_2$.
%\end{proof}
%
%
%
%%\subsection{More about the stabilizer}
%%
%%Let $L$ as before and let $(u_1,u_2)$ be the integer pair associated to $L$. We would like to reformulate Conjecture \ref{conj:Equidistribution of collection of orbits on SU_2^2-quotient} in terms of $\SO_3$. Note that under the natural map $\SU_2 \to \SO_3$ the image of $\SU_2(\Z^S)$ has finite index in $\SO_3(\Z^S)$ (by covolume considerations) and therefore the map
%%\begin{align*}
%%\rquot{\SU_2^2(\Q^S)}{\SU_2^2(\Z^S)} &= \rquot{\SU_2(\Q^S)}{\SU_2(\Z^S)}\times \rquot{\SU_2(\Q^S)}{\SU_2(\Z^S)}\\ 
%%&\to \rquot{\SO_3(\Q^S)}{\SO_3(\Z^S)} \times \rquot{\SO_3(\Q^S)}{\SO_3(\Z^S)} 
%%\\ &= \rquot{\SO_3^2(\Q^S)}{\SO_3^2(\Z^S)}
%%\end{align*}
%%is a finite covering of the image, which is open in the quotient on the right hand side. We would now like to understand the image of the packets constructed earlier. For any $v \in \Z^3$ denote by $\BH_v$ the stabilizer of $v$ in $\SU_2^2$. By Proposition \ref{prop:assoc.int.pairs} we know that
%%\begin{align*}
%%\BH(\Q_S) \subset \BH_{u_1}(\Q_S) \times \BH_{u_2}(\Q_S).
%%\end{align*}
%%
%%\begin{remark}[Remaining question]
%%It would be interesting to know, if equality holds here.
%%\end{remark}
%%
%%By dimensionality reasons, we know that $\BH(\Q_S)$ is an open subgroup of $\BH_{u_1}(\Q_S) \times \BH_{u_2}(\Q_S)$ and therefore any packet is an open subset of an associated packet under $\BH_{u_1}(\Q_S) \times \BH_{u_2}(\Q_S)$. 
%%
%%\begin{remark}[Remaining question]
%%It would be interesting to know, if equality of packets holds here.
%%\end{remark}
%%
%%The latter packets are however mapped into the known packets in the congruence quotient of $\SO_3$ and therefore we can deduce that any limit measure of the invariant measures on our packets is a joining on
%%\begin{align*}
%%\rquot{\SU_2^2(\Q^S)}{\SU_2^2(\Z^S)} &= \rquot{\SU_2(\Q^S)}{\SU_2(\Z^S)}\times \rquot{\SU_2(\Q^S)}{\SU_2(\Z^S)} .
%%\end{align*}
%
%
%
%
%
%
%
%
%
%
%
%\newpage
%We now give an alternative approach for the construction of integer pairs.
%
%\subsection{Spacing properties}
%
%In this section, we will define an $\SO_4(\R)$-invariant metric $d$ on $\Gr(2,4)$ for which we will prove the following estimate:
%
%\begin{proposition}\label{prop:spacing property}
%Let $\Lambda,\Lambda'$ be two rank $2$ sublattices of $\Z^4$ on which the restriction of $Q_0$ has discriminant $D$ and let $L=\text{span}(\Lambda),L' = \text{span}(\Lambda')$. Then
%\begin{align*}
%d(L,L') \gg \frac{1}{\sqrt{D}}.
%\end{align*}
%\end{proposition}
%
%Consider the Pl\"ucker embedding
%\begin{align*}
%\Phi: \Gr(2,4) \to \BP(\wedge^2 \R^4), \quad  \text{span}(v,w) \mapsto v \wedge w
%\end{align*}
%We begin with a few observations:
%\begin{itemize}
%\item The Pl\"ucker embedding is clearly well-defined, since any change of basis will only result in changing the image by an (irrelevant) factor, the determinant of the transformation matrix.
%\item $\Phi$ is an injective map and its image is exactly the set of pure wedges.
%\item As $\Phi$ is continuous, it defines a homeomorphism onto its image.
%\end{itemize}
%The map $v \wedge w \mapsto gv \wedge gw$ for $g \in \SO_4(\R)$ defines an action of $\SO_4(\R)$ on pure wedges (that is, the image of $\Phi$) and clearly extends to an action on $\wedge^2 \R^4$. In what follows, we usually identify $\wedge^2 \R^4 = \R^6$.
%
%\begin{claim}
%The standard norm on $ \R^6$ is invariant for the action of $\SO_4(\R)$ defined above.
%\end{claim}
%
%\begin{proof}
%A computation.
%\end{proof}
%
%The action of $\SO_4(\R)$ on $\R^6$ descends to an action on $\BP(\R^6)$. Naturally, $\Phi$ is equivariant for this action. Given two lines in $\BP(\wedge^2 \R^4)$ their distance is defined as the distance of their norm one elements. In particular, we obtain an $\SO_4(\R)$-invariant metric on $\Gr(2,4)$ by equivariance of $\Phi$.
%
%We say that $L \in \Gr(2,4)$ is \textbf{integral}, if it is spanned by a rank two sublattice of $\Z^4$. It is \textbf{primitive}, if it is spanned by a primitive lattice. Analogously, an integral structure for points in $\BP(\wedge^2 \R^4) = \BP(\R^6)$ and a notation of primitivity is attained. 
%
%\begin{lemma}
%Let $L \in \Gr(2,4)$. If $L$ is integral then $\Phi(L)$ is integral and the same applies to primitivity.
%\end{lemma}
%
%\begin{proof}
%If $L$ is integral, then certainly $\Phi(L)$ is also integral. Assume that $L$ is primitive. Then let $v_1,v_2$ be a $\Z-$basis of $L$ and consider the matrix $g = (v_1|v_2)$. By primitivity of $L$ the greatest common divisior of all determinants of 2-by-2 submatrices of $g$ is one. In particular, $\Phi(L)$ is primitive.
%\end{proof}
%
%We claim that the discriminant corresponds to the length of an integer point under the Pl\"ucker embedding. More precisely,
%
%\begin{claim}
%Let $\Lambda < \Z^4$ be a rank two sublattice so that $\disc(Q_0,\Lambda) = D$. Then the covolume of $\Lambda$ in $L= \text{span}(\Lambda)$ is $ \sqrt{D}$. Furthermore, $\Phi(L)$ is spanned by an integer point of norm $\sqrt{D}$.
%\end{claim}
%
%\begin{proof}
%For the first statement: Let $v_1,v_2$ be a basis of $\Lambda$, write $g = (v_1,v_2)$ and choose $k \in \SO_4(\R)$ so that $kL \subset \R^2 \times \set{(0,0)}$. Then note that $kg$ is of the form $\left(\begin{array}{c}
%\bar{g} \\ 
%0
%\end{array} \right)$for $\bar{g} \in \GL_2(\R)$ and compute
%\begin{align*}
%D = \det(g^t g) = \det(g^tk^t kg) = \det(\bar{g}^t\bar{g}) = \det(\bar{g})^2.
%\end{align*}
%Observe that $\det(\bar{g})$ is the covolume of $\Lambda$ to conclude. To the second statement: the line $\Phi(L)$ is spanned by the primitive vector $v_1 \wedge v_2$. In the previous notation we obtain
%\begin{align*}
%\norm{v_1 \wedge v_2} = \norm{kv_1 \wedge kv_2} = \norm{ \det(\bar{g})e_1\wedge e_2} = \sqrt{D}
%\end{align*}
%\end{proof}
%
%\begin{proof}[Sketch of proof of Proposition \ref{prop:spacing property}]
%By definition of the metric on $\Gr(2,4)$ it suffices to estimate the distance of $\Phi(L)$ and $\Phi(L')$. This can be done efficiently using the fact that integer points are one apart.
%\end{proof}

%
%
%
%\newpage
%\subsection{Using equidistribution of integer points}
%
%\begin{lemma}
%The collections $\tilde{\mathcal{O}}_D$ are equidistributed in $\rquot{\SO_3(\Q_S)}{\SO_3(\Z^S)} = \tilde{X}_S$. 
%\end{lemma}
%
%\begin{proof}
%Let $\mu$ be any \wstar -limit of the sequence $\tilde{\mu}_D$. By REF $\mu$ satisfies 
%\begin{align*}
%(\pi_p)_*\mu = m_{X_p}, \quad (\pi_q)_*\mu = m_{X_q},
%\end{align*}
%where
%\begin{align*}
%\tilde{X}_p = \rquot{\SO_3(\Q_{\set{\infty,p}})}{\SO_3(\Z^{\set{\infty,p}})}, \quad
%\tilde{X}_q = \rquot{\SO_3(\Q_{\set{\infty,q}})}{\SO_3(\Z^{\set{\infty,q}})}
%\end{align*}
%and $\pi_p: \tilde{X}_S \to \tilde{X}_p$, $\pi_q: \tilde{X}_S \to \tilde{X}_q$ denote the projections. Let $a_q$ be a diagonalizable element in $\SO_3(\Q_S)$ under which $\mu$ is invariant. We foliate the measure $\mu$ along the projection $\pi_p$: Let $\mathcal{C}_p$ be the preimage of the Borel $ \sigma$-algebra on $\tilde{X}_p$ under $\pi_p$ and consider the conditional measures $\mu_x^{\mathcal{C}_p}$ for $\mathcal{C}_p$. Let $C$ be a co-null set in $ \tilde{X}_S$ such that the conditional measures are defined for all $x \in C$. Note that the conditional measure $\mu_x^{\mathcal{C}_p}$ for $x \in C$ is supported on an $\SO_3(\Z_q)$-orbit in $ \tilde{X}_S$. Furthermore, we have
%\begin{align*}
%\mu = \int \mu_x^{\mathcal{C}_p} d\mu(x)
%\end{align*}
%for all $x\in C$. Therefore, 
%\begin{align*}
%m_{\tilde{X}_q} = (\pi_q)_* \mu = \int (\pi_q)_*\mu_x^{\mathcal{C}_p} d\mu(x).
%\end{align*}
%Now for any $k \in \SO_3(\Z_q)$ we have 
%\begin{align*}
%\int (\pi_q)_*\mu_x^{\mathcal{C}_p} d\mu(x) = m_{\tilde{X}_q} = k_* m_{\tilde{X}_q} = \int k_* (\pi_q)_* \mu_x^{\mathcal{C}_p} d\mu(x) = \int (\pi_q)_* k_* \mu_x^{\mathcal{C}_p} d\mu(x) 
%\end{align*}
%and so by uniqueness of decomposition\note{This is not true as it stands.} $ (\pi_q)_*k_* \mu_x^{\mathcal{C}_p} = (\pi_q)_*\mu_x^{\mathcal{C}_p} $. However, as both measures are supported on the $\SO_3(\Z_q)$-orbit through $x$, we may eliminate the projection from this equality to obtain invariance. In fact, let $B \subset \tilde{X}_S$ measurable and choose $B'$ so that $B \cap \SO_3(\Z_q) = \pi_q^{-1}B'$ and compute
%\begin{align*}
%\mu_x^{\mathcal{C}_p}(B) = \mu_x^{\mathcal{C}_p}(B \cap x\SO_3(\Z_q)) = (\pi_q)_*\mu_x^{\mathcal{C}_p}(B') = (\pi_q)_*k_* \mu_x^{\mathcal{C}_p}(B') = k_* \mu_x^{\mathcal{C}_p}(B).
%\end{align*}
%Therefore, $k_* \mu_x^{\mathcal{C}_p} = \mu_x^{\mathcal{C}_p}$ as claimed. In particular, $\mu$ is $k$-invariant and thus $\SO_3(\Z_q)$-invariant. However, $\SO_3(\Z_q)$-invariant measures on $\tilde{X}_S$ correspond via the projection $\pi_p$ one-to-one to measures on $\tilde{X}_p$, where the push-forward of $\mu$ is the Haar measure. Therefore, $\mu$ was the Haar measure to start with.
%\end{proof}

\section{The joinigs theorem}

\begin{lemma}
Let $\G$ and $\G'$ be two semisimple algebraic groups defined over $\Q$. Let $\mathbb{M} < \G\times \G'$ be a non-trivial $\Q$-subgroup, which projects onto both components surjectively. Then the adjoint forms of $\G$ and $ \G'$ are equal.
\end{lemma}

\begin{proof}
Assume that $\G,\G'$ are almost simple. Let $\Fm$, $\Fg$, $\Fg'$ be the Lie-algebra of $\BM,\BG,\BG'$ respectively. Denote by $\pi:\BM \to \BG$, $\pi': \BM  \to \BG'$ the respective projections and let $F: \Fm \to \Fg$, $F': \Fm \to \Fg'$ their derivatives (which are defined over $\Q$). Then for any $g\in \BM$ we have $\Ad_{\pi(g)}  \circ F = F \circ \Ad_g$. Assume for a moment that $F$ is an isomorphism. Then the map
\begin{align*}
\Ad(\BM) \to \Ad(\G),\quad \Ad_g \mapsto F \circ \Ad_g \circ F^{-1}
\end{align*}
is a well-defined $\Q$-isomorphism. The fact that $F$ is indeed an isomorphism follows from the non-triviality assumption on $\BM$ and the following claim.
\end{proof}

\begin{claim*}
Let $\Fg,\Fg'$ be simple Lie algebras and let $\Fm$ be a subalgebra of $\Fg \oplus \Fg'$, which projects surjectively onto both components. Then $\Fm$ is either the graph of an isomorphism from $\Fg$ to $\Fg'$ or $\Fm = \Fg \oplus \Fg'$.
\end{claim*}

\begin{proof}
Let $\pi:\Fm \to \Fg$ and $\pi': \Fm \to \Fg'$ the respective projections. Then
\begin{align*}
\Fg' \isom \rquot{\Fm}{\ker(\pi')} \overset{\sim}{\longrightarrow} \rquot{\Fg}{\pi(\ker(\pi'))}
\end{align*}
yields that $\pi(\ker(\pi'))$ is an ideal of $\Fg$. Analogously, one verifies that $\pi'(\ker(\pi))$ is an ideal of $\Fg'$. We now use simplicity and distinguish cases.
\begin{enumerate}[(i)]
\item If $\pi(\ker(\pi'))= \Fg$, then $\Fm$ contains $\Fg \oplus \set{0}$. But since $\pi': \Fm \to \Fg'$ is surjective, the subalgebra $\Fm$ must also contain $\set{0} \oplus \Fg'$ and hence $\Fm = \Fg \oplus \Fg'$. Analogously, the case $\pi'(\ker(\pi)) = \Fg'$ is treated.
\item Assume that $\pi(\ker(\pi'))= \set{0}$ and $\pi'(\ker(\pi)) = \set{0}$. In particular, since $\pi$ is injective on $\ker(\pi')$, we have $\ker(\pi') = \set{0}$. But $\pi'$ is also surjective and hence $\pi'$ is an isomorphism. Analogously, $\pi$ is an isomorphism and therefore $\Fm$ is the graph of the isomorphism $\pi'\circ \pi^{-1}: \Fg \to \Fg'$. 
\end{enumerate}
\end{proof}

\begin{proposition}
Let $\G$ be a simply-connected, almost simple algebraic group defined over $\Q$. Let $\mathbb{M} < \G^2$ be $\Q$-group, which projects onto both components surjectively. Then $\mathbb{M}$ is either $\G^2$ or the graph under an isomorphism from $\G$ to itself, which is defined over $\Q$. 
\end{proposition}

\begin{proof}
Let $\Fm$, $\Fg$ be the Lie-algebra of $\BM,\BG$ respectively. By the claim above, we first consider the case $\Fm = \Fg \oplus \Fg$. Since $\BG$ is connected, this case is readily dealt with. Assume therefore that the derivative of the projection $\pi: \BM \to \BG$ is an isomorpism. In particular, the projection $\pi: \BM \to \BG$ is a central isogeny by simplicity. But $\BG$ is simply connected and hence $\pi: \BM \to \BG$ is an isomorphism defined over $\Q$. We thus obtain the proposition.
\end{proof}

Recall that any automorphism of $\SU_2$ is inner (see REF Platonov Rapinchuk). We now discuss the effect this has on stabilizer subgroups of integer points.

\begin{lemma}
Let $u,v$ be primitive integer points in $\Z^3$ and assume that there is some $\gamma \in \SU_2(\Q)$, such that $\gamma \BH_v \gamma^{-1} = \BH_u$. Then $\gamma.v$ is equal to $u$ up to a sign.
\end{lemma}

\begin{proof}
If $g \BH_v$, then $\gamma .v = \gamma g. v = ( \gamma g \gamma^{-1}) \gamma.v $ shows that $\gamma g \gamma^{-1}\in \BH_u$ fixes $\gamma.v$. However, any element in $\BH_u$ is of this form by assumption and hence by Witt's theorem $\gamma.v$ is a multiple of $u$. But since the length of $\gamma.v$ is equal to the length of $u$, this multiple is $\pm 1$.
\end{proof}


\section{Counting integral embeddings}

In this section, we aim at showing that for given a primitive binary integral quadratic form $Q$ of discriminant $D$ the number of integral embeddings $ Q \to Q_0 $ can be estimated by $\sqrt{D}$ up to an absolute constant. For this, Siegel's mass formula will be used. Let $M$ be the matrix representation of $Q$ with respect to some basis. The general reference for this chapter is REF Kitaoka.

\begin{theorem}[A special case of Siegel's mass formula]
The number $r(Q_0,Q)$ of primitive integral embeddings $(\Z^2,Q) \to (\Z^4,Q_0)$ is given up to a constant by 
\begin{align*}
\sqrt{D} \times \prod_{p \text{ prime}} d_p
\end{align*}
where the local densities $d_p$ are defined as follows: Let $r_p$ be the number $\frac{1}{2}\rank_p(Q)^2 + \frac{7}{2}\rank_p(Q)$, where $\rank_p(Q)$ denotes the rank of the reduction of $M$ mod $p$. Then $d_p$ is $p^{-r_pk}$ times the number of primitive solutions to 
\begin{align}\label{eq:counting integral embeddings-def local densities}
X^t X = M \mod p^k
\end{align}
for some $k$ large enough (depending on $p$).
\end{theorem}

Note that Siegel's mass formula states the appearing constant explicitly. As we are interested in the growth of the number of solutions only, we chose to omit it. Furthermore, this special case uses the fact that the genus of $Q_0$ consists of one class only.

As Kitaoka mentions on page 100, the fact that the quadratic lattice $(\Z^4,Q_0)$ is unimodular yields that one may consider $k = 1$ in Equation \eqref{eq:counting integral embeddings-def local densities} for odd primes $p$, that is
\begin{align*}
d_p = p^{-5} |\setc{X\in \Mat_{4,2}(\Fp)}{X^tX = \bar{M}}|
\end{align*}
where $\bar{M}$ denotes the reduction of $M$ mod $p$. In the following, we will compute $d_p$ as precisely as possible for an odd prime $p$.

\begin{remark}
Alternatively, we could invoke Theorem 1.3.2 in REF Kitaoka directly. Assume $p \nmid D$ and the notation in Kitaoka. Then $\chi(\bar{Q}) = \chi(x^2+Dy^2) = 1$ if $-D$ is a square and $-1$ otherwise. Also, 
\begin{align*}
\chi(\bar{Q}_0) = \chi(x_1^2+Dx_2^2+x_3^2+Dx_4^2) = 1^2 = 1
\end{align*}
The number of embeddings $(\Fp^2,\bar{Q})\to (\Fp^4,\bar{Q}_0)$ is\note{This has to be verified!!}
\begin{align*}
\left\lbrace\begin{array}{cc}
p^{5}(1-p^{-2})(1+p^{-1}) & \text{if }-D \text{ is a square } \mod p \\ 
p^{5}(1-p^{-2})(1-p^{-1}) & \text{if }-D \text{ is not a square } \mod p
\end{array} \right. .
\end{align*}
We will not use this later.
\end{remark}

\begin{claim}
The equation 
\begin{align}\label{eq:counting integral embeddings-XtX=M}
X^tX = \bar{M}
\end{align}
always has a solution. Equivalently, $d_p$ is positive.
\end{claim}

\begin{proof}
Assume that $\bar{D} \neq 0$ first i.e. $p \nmid D$. In this case, the quadratic form $\bar{Q}$ given by the reduction of $Q$, that is the quadratic form induced by $\bar{M}$ is non-degenerate. By the classification of quadratic forms over $\Fp$, $\bar{Q}$ is equivalent to $x^2+\bar{D}y^2$ and we may just as well find a solution to
\begin{align*}
X^tX = \left(\begin{array}{cc}
1 & 0 \\ 
0 & \bar{D}
\end{array} \right).
\end{align*}
Writing $\bar{D} = \alpha^2+\beta^2$ for $\alpha,\beta\in \Fp$ the matrix 
\begin{align*}
X = \begin{pmatrix}
1 & 0 \\ 
0 & 0 \\ 
0 & \alpha \\ 
0 & \beta
\end{pmatrix} 
\end{align*}
is such a solution. The same approach works if $\bar{D}=0$, since by primitivity of $Q$ we never have $\bar{M}=0$.
\end{proof}

Starting from a given solution to Equation \eqref{eq:counting integral embeddings-XtX=M} we will construct new ones using Witt's theorem. Notice that if $X$ is a solution, then so is $gX$ for any $g\in \GO_4(\Fp)$. Any other solution is of this form:

\begin{lemma}[Transitivity of $\GO_4(\Fp)$-action on solutions]
Let $X,Y$ be another solution to Equation\eqref{eq:counting integral embeddings-XtX=M}. Then there exists an isometry $g \in \GO_4(\Fp)$ with $g X = Y$.
\end{lemma}

\begin{proof}
Write $X = (x_1,x_2)$ and $Y = (y_1,y_2)$ and let $U$ resp. $U'$ be the subspace of $\Fp^4$ spanned by $x_1,x_2$ resp. $y_1,y_2$. The isometry $\phi: U \to U'$ defined by $x_1 \mapsto y_1,\ x_2 \mapsto y_2$ extends by Witt's theorem to an isometry $\Fp^4 \mapsto \Fp^4$.
\end{proof}

Hence we have a transitive action of $\GO_4(\Fp)$ on the set of solutions to \eqref{eq:counting integral embeddings-XtX=M}. We determine the stabilizer of a point: Let $X$ be a solution to \eqref{eq:counting integral embeddings-XtX=M} and assume $p \nmid D$ for a minute. Then the span of the columns of $X$ is a two-dimensional subspace $U$ and the stabilizer $H$ of $X$ is the subgroup of $\SO_4(\Fp)$, whose elements fix $U$ pointwise. In particular, 
\begin{align*}
H \isom \GO_{Q_0|_{U^{\perp}}}(\Fp) \isom \GO_{x^2+\bar{D}y^2}(\Fp).
\end{align*}

TO DO: degenerate case.


We say that a quadratic space is hyperbolic, if it is a sum of hyperbolic planes (in this case, even dimension is automatic).

\begin{example}\label{exp:counting integral embeddings-Q0 hyperbolic}
The quadratic space $(\Fp^4,Q_0)$: if $-1$ is a square, this is obvious. Otherwise, fix some non-square $\alpha$ and see that
\begin{align*}
x_1^2+x_2^2+x_3^2+x_4^2 \simeq x_1^2+x_2^2+ \alpha x_3^2+\alpha x_4^2 \simeq x_1^2+ \alpha x_2^2+x_3^2+ \alpha x_4^2
\end{align*}
This shows that $(\Fp^4,Q_0)$ is the direct sum of two copies of the hyperbolic plane $(\Fp^2,x^2+\alpha y^2)$.
\end{example}

\begin{example}\label{exp:counting integral embeddings-Q hyperbolic?}
The quadratic space $(\Fp^2,\bar{Q})$ for $p \nmid D$ is hyperbolic if and only if $-D$ is a square mod $p$, since $\bar{Q} \simeq x^2+Dy^2$.
\end{example}

In the continuation we shall use the following proposition which gives the cardinality of the orthogonal groups involved. 


\begin{proposition}[REF Wilson]
Let $(V,q)$ be a quadratic space over $\Fp$. Then the orthogonal group $\GO_q(\Fp)$ satisfies
\begin{align*}
|\GO_q(\Fp)| = 2 \prod_{k=1}^m ((p^{2k}-1)p^{2k-1}) = 2 p^{m^2}(p^2-1)(p^4-1)...(p^{2m}-1)
\end{align*}
if $\dim(V) = 2m+1$ is odd and if $\dim(V) = 2m$ and $(V,q)$ is hyperbolic,
\begin{align*}
|\GO_q(\Fp)| = 2p^{m(m-1)} (p^m-1) \prod_{k=1}^{m-1}(p^{2k}-1)
\end{align*}
and
\begin{align*}
|\GO_q(\Fp)| = 2p^{m(m-1)} (p^m+1) \prod_{k=1}^{m-1}(p^{2k}-1)
\end{align*}
otherwise.
\end{proposition}

By Example \ref{exp:counting integral embeddings-Q0 hyperbolic} we deduce ($m=2$)
\begin{align*}
|\GO_4(\Fp)| = 2p^2(p^2-1)^2
\end{align*}
By Example \ref{exp:counting integral embeddings-Q hyperbolic?} we deduce ($m=1$) that for any $p \nmid D$
\begin{align*} |\GO_{x^2+Dy^2}(\Fp)| = 
\left\lbrace \begin{array}{ll}
2(p-1) & \text{ if} -D \text{ is a square } \mod p \\ 
2(p+1) & \text{ if} -D \text{ is not a square } \mod p
\end{array} \right.
\end{align*}
Let $\chi$ be the Kronecker symbol associated to the number field with discriminant $-D$. Then compute (still for $p \nmid D$)
\begin{align*}
d_p = p^{-5} \frac{|\GO_4(\Fp)|}{|\GO_{x^2+Dy^2}(\Fp)|} &= 
\left\lbrace \begin{array}{ll}
p^{-3}(p^2-1)(p+1) & \text{ if } \chi(p) = 1 \\ 
p^{-3}(p^2-1)(p-1) & \text{ if } \chi(p) = -1
\end{array}\right. \\
&=
\left\lbrace \begin{array}{ll}
(1-p^{-2})(1+p^{-1}) & \text{ if } \chi(p) = 1 \\ 
(1-p^{-2})(1-p^{-1}) & \text{ if } \chi(p) = -1
\end{array}\right.\\
&=\left\lbrace \begin{array}{ll}
(1-p^{-2})^2(1-p^{-1})^{-1} & \text{ if } \chi(p) = 1 \\ 
(1-p^{-2})^2(1+p^{-1})^{-1} & \text{ if } \chi(p) = -1
\end{array}\right.\\ 
&= (1-p^{-2})^2 \frac{1}{(1-\chi(p)p^{-1})}
\end{align*}
For an odd prime $p$ with $p | D$ the cardinality of the stabilizer of a solution $X$ to \eqref{eq:counting integral embeddings-XtX=M} is $2p(p^2-1)$. We obtain
\begin{align*}
d_p = p^{-3} \frac{2p^2(p^2-1)^2}{2p(p^2-1)} = 1-p^{-2} = (1-p^{-2})^{-1} \frac{(1-p^{-2})^2}{(1-\chi(p)p^{-1})}
\end{align*}
Overall, $\prod_p d_p$ is up to a constant
\begin{align*}
\prod_p \frac{(1-p^{-2})^2}{(1-\chi(p)p^{-1})} = \frac{L(1,\chi)}{\zeta(2)^2}
\end{align*}
By Siegel's lower bound we obtain

\begin{proposition}
The number of primitive integral embeddings $(\Z^2,Q) \to (\Z^4,Q_0)$ is $\gg_\varepsilon D^{\frac{1}{2}-\varepsilon}$.
\end{proposition}









%
%In the following, we find a lower bound for $\alpha_p$, where $p$ is an odd prime. To do so, we apply Lemma 1.7 in REF my paper and hence distinguish the following cases where $-D$ is a square mod $p$ and where it isn't.
%
%\subsection{-D is a square mod p}
%
%Assume that $-D$ is a square mod $p$. By Lemma 1.7 in REF it suffices to count the number of solutions to
%\begin{align}\label{eq:counting integral embeddings- -D square1}
%X^t X = \begin{pmatrix}
%0 & 1 \\ 
%1 & 0
%\end{pmatrix}  \mod p^k.
%\end{align}
%Note already that this number does not depend on $D$ and only consists of three polynomial equations to be solved simultaneously. We would like to use the following result by Warning to compute the number of solutions for $k=1$.
%
%\begin{theorem}[Warning's theorem]
%Let $n,d_1,...,d_r$ be positive integers with $d_1+...+d_r < n$ and for any $i$ let $f_i(t_1,...,t_n) \in \Fp[t_1,...,t_n]$ be a polynomial of total degree $d_i$. Then the number of common zeros of the $f_i$'s on $\Fp^n$ is divisible by $p$.
%\end{theorem}
%
%An exposition of Warning's theorem may be found in REF Clark(e). The original paper is REF. We rewrite Equation \eqref{eq:counting integral embeddings- -D square1} for $k=1$ as
%\begin{align}
%x_1^2+x_2^2+x_3^2+x_4^2 = 0  \label{eq:counting integral embeddings- -D square2.1} \\
%y_1^2+y_2^2+y_3^2+y_4^2 = 0  \label{eq:counting integral embeddings- -D square2.2}\\
%x_1y_1+x_2y_2+x_3y_3+x_4y_4 = 1  \label{eq:counting integral embeddings- -D square2.3}
%\end{align}
%over $\Fp$ where we wrote
%\begin{align*}
%X = \begin{pmatrix}
%x_1 & y_1 \\ 
%x_2 & y_2 \\ 
%x_3 & y_3 \\ 
%x_4 & y_4
%\end{pmatrix} .
%\end{align*}
%By Warning's theorem the set of solutions $\mathcal{S}$ to Equations \eqref{eq:counting integral embeddings- -D square2.1},\eqref{eq:counting integral embeddings- -D square2.2},\eqref{eq:counting integral embeddings- -D square2.3} has a cardinality divisible by $p$. TO DO: a solution exists.
%
%
%\begin{claim}
%If $X$ is a solution, then so is $Xg$ for any $g \in \GL_2(\Fp)$ of the form
%\begin{align*}
%g = \begin{pmatrix}
%a & 0 \\ 
%0 & a^{-1}
%\end{pmatrix}, a \in \Fp^\times.
%\end{align*}
%\end{claim}
%
%The proof is a straightforward computation. In particular, $|\mathcal{S}|$ is divisible by $p-1$ and since $\gcd(p,p-1) = 1$ we have that $p(p-1)$ divides $|\mathcal{S}|$.
%




%Equation \eqref{eq:counting integral embeddings- -D square2.3} is equivalent to
%\begin{align*}
%x_1y_1+x_2y_2+x_3y_3 -1 = x_4y_4 
%\end{align*}
%from which we may eliminiate $x_4$ and $y_4$ by using Equations \eqref{eq:counting integral embeddings- -D square2.1} and \eqref{eq:counting integral embeddings- -D square2.2}. This yields 
%\begin{align}\label{eq:eq:counting integral embeddings- -D square3}
%(x_1y_1+x_2y_2+x_3y_3 -1)^2 = (x_1^2+x_2^2+x_3^2)(y_1^2+y_2^2+y_3^2)
%\end{align}
%Let $\mathcal{S} = \setc{(x_1,x_2,x_3,y_1,y_2,y_3) = (x,y)}{(x,y) \text{ solves } \eqref{eq:eq:counting integral embeddings- -D square3}}$ and note that $p$ divides $ |\mathcal{S}|$ by Warning's theorem. Furthermore, the operations $(x,y) \mapsto (-x,y)$ and $(x,y) \mapsto (x,-y)$ preserve $\mathcal{S}$ and thus $|\mathcal{S}|$ is also divisible by four.\note{At this point one should explain why no information was lost by squaring.}
%We now claim that ``many'' points $(x,y)$ in $\mathcal{S}$ satisfy that $-(x_1^2+x_2^2+x_3^2)$ and $-(y_1^2+y_2^2+y_3^2)$ are squares. First of all, note that if $-(x_1^2+x_2^2+x_3^2)$ is a square, then the same holds for $-(y_1^2+y_2^2+y_3^2)$ by Equation \eqref{eq:eq:counting integral embeddings- -D square3}.

\begin{appendix}

\section{Miscellaneous}

\subsection{A basis for the lattice}
Let $Q$ and $\iota_Q$ be as before and set $L := \iota_Q(\Z^2)$ for simplicity.
\begin{lemma}\label{lemma:orbital-setup lattice maximal}
The lattice $L \subset \Z^4$ is a maximal rank $2$ sublattice. In particular, any basis consists of primitive vectors.
\end{lemma}

Notice that the lemma implies the recovering lemma.

\begin{proof}
Suppose that there is a rank $2$ lattice $L'$ which strictly contains $L$. Represent $Q_0|_{L'}$ by a matrix $M \in \Mat_2(\Z)$. By assumption there exists $g \in \Mat_2(\Z)$ so that 
\begin{align*}
g^t M g = M_Q
\end{align*}
where $M_Q$ represents $Q$ on $\Z^2$. This contradicts the assumption that $D = \det(M_Q)$ is square-free.\note{Morally, primitivity should be enough.}
\end{proof}

\begin{proposition}
There is a basis $v_1,v_2$ of $L$, $w_1,w_2 \in \Z^4$ and $u_1,u_2$ a basis of $L^\perp \cap \Z^4$ so that
\begin{align*}
g_L := (u_1,u_2,w_1,w_2) \in \SL_4(\Z).
\end{align*}
and $(w_i,v_i) = 1$ for $i=1,2$. 
\end{proposition}

\begin{proof}
Let $v_1,v_2$ be a basis of $L$ and note that $v_1,v_2$ are automatically primitive. Denote $g = (v_1,v_2)$. Apply the elementary divisor theorem to obtain $S \in \SL_4(\Z)$ and $T \in \SL_2(\Z)$ such that
\begin{align*}
SgT = \begin{pmatrix}
\alpha_1 &  \\ 
 & \alpha_2 \\ 
 &  \\ 
 & 
\end{pmatrix} = g'
\end{align*}
with $\alpha_1 | \alpha_2$. By primitivity of $v_1,v_2$ we have $\alpha_1 = 1$. We claim that $\alpha_2 = 1$: Let $L' = T^{-1}\Z^2$ and note that $gTL' = L$. If $\alpha_2 \neq 1$, then $L$ is not maximal as
\begin{align*}
L = gTL' = S^{-1}g' L' \subset S^{-1} \begin{pmatrix}
1 &  \\ 
 & 1 \\ 
 &  \\ 
 & 
\end{pmatrix} L'
\end{align*}
is a strict inclusion.\note{In particular, there exists an invertible matrix with $v_1,v_2$ in the first two rows.} Set $v_i = gTe_i \in L$, $w_i = S^t e_i$ and $u_i = S^t e_{i+2}$ for $i = 1,2$. Compute
\begin{align*}
(w_i,v_i) = e_i^t g' e_i = 1, \quad (u_i,v_j) = ... =  0.
\end{align*}
This implies that $u_1,u_2$ is a basis of $L^t \cap \Z^4$.
\end{proof}

Observe that the element $g_L$ in the proposition is unique up to a factor in
\begin{align*}
\left(\begin{array}{c|c}
\SL_2 & \Mat_2 \\ 
\hline
0 & I_2
\end{array} \right) < \SL_4
\end{align*}
on the right.

%\subsection{Orthogonal lattice}
%
%Fix $Q$ and $\iota_Q$ as above and denote for simplicity $\Lambda := \Lambda_{Q,\iota_Q} := \iota_Q(\Z^2)^\perp \cap \Z^4$. Choose $k_Q \in \SO_4(\R)$ so that 
%\begin{align*}
%k_Q \iota_Q(\Z^2) \subset \R^2 \times \set{(0,0)} 
%\end{align*}
%We thus also have $k_Q \Lambda  \subset \set{(0,0)} \times \R^2$. Let $a_Q$ be a diagonal matrix which commutes with $K:= \SO_2(\R) \times \SO_2(\R)$ and so that $a_Q k_Q \Lambda$ is unimodular.\note{To be chosen concretely.} Recalling that $k_Q$ is unique up to a choice in $K$, we obtain a point $x_{Q,\iota_Q}$ in the space
%\begin{align*}
%\lrquot{\SO_2(\R)}{\SL_2(\R)}{\SL_2(\Z)} = \rquot{\mathbb{H}}{\SL_2(\Z)} =: Y.
%\end{align*}
%Denote
%\begin{align*}
%\mathcal{S}'_D = \setc{(P_{Q,\iota_Q},x_{Q,\iota_Q})}{P_{Q,\iota_Q} \in \mathcal{S}_D}.
%\end{align*}
%
%\begin{conjecture}[Simultaneous equidistribution]
%Under the congruence conditions in Conjecture \ref{conj:equidistribution of planes} the sets $\mathcal{S}_D'$ equidistribute to the Haar measure on $X \times Y$.
%\end{conjecture}

\end{appendix}

==> squaring.tex <==
\showthesis{
\newpage
\section{Squaring in the class group}

In this section we briefly explain a somewhat complementary argument for the equidistribution of the sets
\begin{align*}
\setc{(\tfrac{1}{\sqrt{D}} v,[\Lambda_v])}{v \in \Z^3 \text{ with } Q(v) = D } \subset 
\mathbb{S}^2 \times \mathcal{CM}_D
\end{align*}
to the one given in \cite{AES3D}. Here, $D \in \mathbb{D}$ is square-free.
To do so, let us first the action of the class group on the set above.

\begin{lemma}\label{lemma:squaring}
For any $[\Fa]\in \Cl(\mathcal{O}_D)$ we have $[\Lambda_{[\Fa].v}] = [\Fa]^2.[\Lambda_v]$.
\end{lemma}

This follows from the results in Section 5.2 in \cite{Linnikthmexpander}, but we would like to provide a direct argument here.
The way to access the action of the class group is via the adelic viewpoint. 
Define the $\Q$-group $\mathbb{H}$ as the group obtained by projectivizing the restriction of scalars of $\G_m$ for $K$ over $\Q$.
More explicitly, one may define $\BH$ for our purposes here as the stabilizer $\BH_{q}$ in $\PGL_2$ of a binary form $q$ of discriminant~$D$.\awnote{$\PGL_2$ or $\SL_2$?}
Then the class group of $K$ is isomorphic to the double quotient
\begin{align*}
\Cl(\BH) := \lrquot{\BH(\Q)}{\BH(\adele_f)}{\BH(\widehat{\Z})},
\end{align*}
see for instance \cite[Sec.8.3]{Linnikthmexpander} or \cite[Prop.3.5]{W18}.

Recall that for any two binary forms $q,q'$ there is a natural isomorphism $\Cl(\BH_{q}) \cong \Cl(\BH_{q'})$ defined as follows.
Choose $\gamma\in \PGL_2(\Q)$ and $g \in \PGL_2(\R\times \widehat{\Z})$ with $\gamma.q = g.q = q'$. Then
\begin{align*}
\Cl(\BH_q) \ni \BH_{q}(\Q)h \BH_{q}(\R \times \widehat{\Z}) \mapsto 
\BH_{q'}(\Q)(\gamma h g^{-1}) \BH_{q'}(\R \times \widehat{\Z})
\in \Cl(\BH_{q'}).
\end{align*}
By the choices of $\gamma$ and $g$ this map is a well-defined isomorphism.
Furthermore, any different choice for $\gamma$ or $g$ yields the same isomorphism.

Notice that any pure quaternion $v\in \quat_0$ yields an embedding of $\Q(\sqrt{-D})$ into $\quat$ and therefore an isogeny
\begin{align*}
\BH \to \Stab_{\SO_3}(v) =: \BH_v.
\end{align*}
The class group $\Cl(\BH_v)$ of $\BH_v$ acts transitively on the set of integer points of norm $\sqrt{D}$ and therefore also $\Cl(\mathcal{O}_D)$ acts transitively as $\Cl(\BH_v)$ is a quotient of $\Cl(\BH)$  (see \cite[Sec.8.3]{Linnikthmexpander}).
In fact, the action of $\Cl(\BH)$ is defined in this fashion.
In the following we would like to understand the map
\begin{align*}
[h]\in \Cl(\BH) \twoheadrightarrow \Cl(\BH_v) \mapsto [h|_{\Lambda_v}] \in \Cl(\BH_{q_v}) \cong \Cl(\BH)
\end{align*}
and more precisely show that it is exactly the squaring map.

\begin{example}[Totally split case]
Let us begin explaining the above phenomenon in a simple special case along the lines of the above. Let $A < \PGL_2$ be the diagonal torus and consider the action of $\PGL_2$ on its Lie algebra via the adjoint.
This action preserves the determinant and hence $\PGL_2 \cong \SO_{\det = x^2-yz}$ via the basis
\begin{align*}
v = \begin{pmatrix}
1 & 0 \\ 
0 & -1
\end{pmatrix} ,w_1 = \begin{pmatrix}
0 & 1 \\ 
0 & 0
\end{pmatrix}, w_2 = 
\begin{pmatrix}
0 & 0 \\ 
1 & 0
\end{pmatrix}.
\end{align*}
This basis also decomposes the action of $A$ into eigenspaces, where the span of $v$ is the trivial eigenspace.
Restricting the action of an element
\begin{align*}
a = \begin{pmatrix}
t & 0 \\ 
0 & 1
\end{pmatrix} \in A
\end{align*}
to the linear span of $w_1,w_2$ (the orthogonal complement of $v$) yields (since the eigenvalue of $a$ on $\langle w_1 \rangle$ is $t$ and on $\langle w_2 \rangle$ is $t^{-1}$)
\begin{align*}
\begin{pmatrix}
t & 0 \\ 
0 & t^{-1}
\end{pmatrix} =  
\begin{pmatrix}
t^2 & 0 \\ 
0 & 1
\end{pmatrix}
\in A = \Stab_{q_v} < \PGL_2
\end{align*}
where $q_v$ denotes the restriction of the determinant to $\Z w_1 \oplus \Z w_2$.
\end{example}

\begin{proof}[Proof of Lemma \ref{lemma:squaring}]
Inspired by the above example we begin by fixing an element $a \in \BH < \PGL_2$ and denote its eigenvalues (possibly in an algebraic closure) by $t,1,t^{-1}$. 
Let $\psi(a)$ be its image in $\BH_v< \SO_3$ again with eigenvalues $t,1,t^{-1}$ for the action on the Lie algebra $\quat_0$ of $\SO_3$.
Here, observe that the eigenvalue $1$ exactly arises on the subspace spanned by $v$.
The restriction of $\psi(a)$ to the orthogonal complement of $v$ (in any basis) yields a two-by-two matrix $\varphi(a)$ with eigenvalues $t,t^{-1}$ (for the action on two-space).
Therefore, the eigenvalues of $\varphi(a)\in \PGL_2$ for the action on the Lie algebra are $t^2,1,t^{-2}$.

In other words, we have shown that the homomorphism
\begin{align*}
\varphi: \BH \to \BH_{q_v}
\end{align*}
defined over $\Q$ maps an element in $\BH$ to an element with squared eigenvalues. Note that there exists some $\gamma \in \GL_2(\Q)$ which conjugates $\BH_{q_v}$ to $\BH$. The above implies that
\begin{align*}
\tilde{\varphi}:\BH \to \BH,\ h \mapsto \gamma \varphi(h) \gamma^{-1}
\end{align*}
is equal to the squaring map $\BH \to \BH,\ h \mapsto h^2$. In particular,
\end{proof}


\begin{lemma}[Bound on $2$-torsion]
Let $K/\Q$ be a quadratic extension, let $\mathcal{O}_K$ be the ring of integers in $K$ and denote by $\Cl(\mathcal{O}_K)[2]$ the $2$-torsion of the class group.
Then
\begin{align*}
|\Cl(\mathcal{O}_K)[2]| \ll_{\varepsilon} \disc(\mathcal{O}_K)^\varepsilon 
\end{align*} 
for any $\varepsilon>0$.
\end{lemma}

The analogous statement holds true for the Picard group.
In terms of quadratic forms the right reference is \cite[Sec.~14.4]{cassels}. In the case of maximal orders a good reference is also \cite[Thm.~39,41]{froehlichtaylor}.

\begin{proof}
Let $[\Fa] \in \Cl(\mathcal{O}_K)$ be of order $2$ and denote by $\overline{\cdot}$ the non-trivial Galois-automorphism of $K/\Q$.

Then the ideal $\frac{\Fa}{\overline{\Fa}}$ satisfies $\frac{\Fa}{\overline{\Fa}} = \frac{\Fa^2}{\Fa\overline{\Fa}}$ and is thus principal.
Write $\frac{\Fa}{\overline{\Fa}} = (\alpha)$ and note that $\Nr(\alpha) =1$.
By Hilbert's theorem 90 there is $\beta\in K$ with $\alpha = \frac{\overline{\beta}}{\beta}$.
Replacing $\Fa$ by $\beta\Fa$ we may thus assume that $\Fa = \overline{\Fa}$.

Now factorize the ideal $\Fa$ into prime ideals as
\begin{align*}
\Fa = \mathfrak{p}_1^{\ell_1} \cdots \mathfrak{p}_k^{\ell_k}
\end{align*}
Since $\Fa = \overline{\Fa}$, any prime $\mathfrak{p}_i$ for which $\mathfrak{p}_i \neq \overline{\mathfrak{p}_i}$ (i.e. for which the underlying rational prime is split) must satisfy $\mathfrak{p}_i = \overline{\mathfrak{p}_j}$ for some $j \neq i$ and $\ell_i = \ell_j$.
We may thus assume  by replacing $\Fa$ in its ideal class that all primes appearing in the above decomposition have an underlying prime which is ramified and more precisely that
\begin{align*}
\Fa = \mathfrak{p}_1 \cdots \mathfrak{p}_k
\end{align*}
where $\mathfrak{p}_i \cap \Z$ is a ramified prime ideal for all $i$.

Conversely, any ideal class, which can be represented in this form, is an order two element
We have shown that $|\Cl(\mathcal{O}_K)[2]|$ is equal to the number of ramified primes $p \in \N$. Now recall that $p \in \N$ is ramified if and only if $p \mid \disc(\mathcal{O}_K)$.
Since the number of divisors $d(D)$ of any $D \in\Z$ is bounded as $d(D) \ll_\varepsilon D^\varepsilon$ for any $\varepsilon>0$, we are done.
\end{proof}

\begin{lemma}[An instance of Hilbert's theorem 90]
Let $\BK$ be a field and let $A \in \SL_2(\BK)$  be diagonalizable. Then there exists $B \in \GL_2(\BK)$ with $[B]^2 = [A]$ in $\PGL_2(\BK)$.
\end{lemma}

\begin{proof}
Denote by $\mathbf{T}$ the centralizer of $A$ in $\Mat_2$ and write $A = g \diag(\lambda,\lambda^{-1})g^{-1}$ where $\lambda$ is an element of a quadratic extension $\BL$ of $\BK$ and $g \in \GL_2(\BL)$.
Denote by $\sigma$ the non-trivial element of $\operatorname{Gal}(\BL/\BK)$ and set
\begin{align*}
B = g \diag(\lambda,1) g^{-1} \in \GL_2(\BL).
\end{align*}
Clearly, $B$ satisfies $[B]^2 = [A]$ in $\PGL_2(\BK)$. It remains to show that $[B] \in \PGL_2(\BK)$.

To see this, observe first that
\begin{align*}
\sigma(B) 
&= \sigma(g) \diag(\lambda^{-1},1)\sigma(g)^{-1}
=\sigma(g) k \diag(1,\lambda^{-1})k^{-1}\sigma(g)^{-1}\\
&\equiv  \sigma(g) k \diag(\lambda,1)k^{-1}\sigma(g)^{-1}
= (\sigma(g) k g^{-1}) B (g k^{-1}\sigma(g)^{-1})
\end{align*}
where $k\in \GL_2(\BK)$ is such that $\diag(\lambda^{-1},1)= k \diag(1,\lambda^{-1})k^{-1}$.
We claim that $\tilde{g} = (\sigma(g) k g^{-1}) \in \GL_2(\BK)$ commutes with $B$, which would prove the lemma.
Since the centralizer of $B$ is equal to the centralizer $\mathbf{T}$ of $A$, it suffices to show this for $A$.
We thus compute
\begin{align*}
\tilde{g} A \tilde{g}^{-1}
&= \sigma(g) k \diag(\lambda,\lambda^{-1})k^{-1}\sigma(g)^{-1}
= \sigma(g) \diag(\lambda^{-1},\lambda)\sigma(g)^{-1}\\
&= \sigma (g \diag(\lambda,\lambda^{-1})g^{-1})
= \sigma(A) =A.
\end{align*}
This concludes the proof of the lemma.
\end{proof}



}

